Improved matrix algorithms via the Subsampled Randomized Hadamard Transform

Several recent randomized linear algebra algorithms rely upon fast dimension reduction methods. A popular choice is the Subsampled Randomized Hadamard Transform (SRHT). In this article, we address the efficacy, in the Frobenius and spectral norms, of an SRHT-based low-rank matrix approximation technique introduced by Woolfe, Liberty, Rohklin, and Tygert. We establish a slightly better Frobenius norm error bound than currently available, and a much sharper spectral norm error bound (in the presence of reasonable decay of the singular values). Along the way, we produce several results on matrix operations with SRHTs (such as approximate matrix multiplication) that may be of independent interest. Our approach builds upon Tropp's in "Improved analysis of the Subsampled Randomized Hadamard Transform".

==> basicincludes.tex <==
\usepackage{graphicx}
\usepackage{amssymb,bm}
\usepackage{setspace}
\usepackage{multirow}
\usepackage{colonequals}
\usepackage{enumerate}

\evensidemargin=0in
\oddsidemargin=0in
\textwidth=6.5in
\topmargin=-0.33in
\headheight=0.25in
\textheight=9in

\renewcommand{\star}{*}

%\newcommand{\mat}[1]{\ensuremath{\bm{#1}}}
\renewcommand{\vec}[1]{\ensuremath{\bm{#1}}}
%\newcommand{\e}{\ensuremath{\mathrm{e}}}
%\newcommand{\E}{\ensuremath{\mathbb{E}}}
%\newcommand{\Prob}[1]{\ensuremath{\mathbb{P}\left(#1\right)}}
\newcommand{\CondProb}[2]{\ensuremath{\mathbb{P}\left\{#1 \,\left|\, #2 \right.\right\}}}
\newcommand{\lnorm}[2]{\ensuremath{\left\| #2 \right\|_{L_{#1}}}}
%\newcommand{\R}{\ensuremath{\mathbb{R}}}
%\newcommand{\C}{\ensuremath{\mathbb{C}}}
\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\N}{\ensuremath{\mathbb{N}}}
\newcommand{\randcon}{\ensuremath{\mathrm{R}}}
\newcommand{\indicator}[1]{\ensuremath{\mathbb{1}\left\{#1\right\}}}
\newcommand{\const}[1]{\ensuremath{\mathrm{#1}}}

%\newcommand{\norm}[1]{\ensuremath{\big\|#1\big\|}}
\newcommand{\F}{F}

\newcommand{\lambdamin}[1]{\ensuremath{\lambda_{\mathrm{min}}\left(#1\right)}}
\newcommand{\sigmamin}[1]{\ensuremath{\sigma_{\mathrm{min}}\left(#1\right)}}
\newcommand{\Isom}[2]{\ensuremath{V_{#1}(\C^{#2})}}
\DeclareMathOperator{\tr}{tr}
%\DeclareMathOperator{\rank}{rank}
\newcommand{\trexp}[1]{\ensuremath{\tr\exp\left(#1\right)}}
%\newcommand{\diag}[1]{\ensuremath{\operatorname{diag}\left(#1\right)}}

%\newtheorem{thm}{Theorem}
\newtheorem{prop}{Proposition}
%\newtheorem{lemma}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{defn}{Definition}
\theoremstyle{remark}
\newtheorem{remark}{Remark}
